Quantitative Separation Logic - A Logic for Reasoning about Probabilistic Programs

We present quantitative separation logic ($\mathsf{QSL}$). In contrast to classical separation logic, $\mathsf{QSL}$ employs quantities which evaluate to real numbers instead of predicates which evaluate to Boolean values. The connectives of classical separation logic, separating conjunction and separating implication, are lifted from predicates to quantities. This extension is conservative: Both connectives are backward compatible to their classical analogs and obey the same laws, e.g. modus ponens, adjointness, etc. Furthermore, we develop a weakest precondition calculus for quantitative reasoning about probabilistic pointer programs in $\mathsf{QSL}$. This calculus is a conservative extension of both Reynolds' separation logic for heap-manipulating programs and Kozen's / McIver and Morgan's weakest preexpectations for probabilistic programs. Soundness is proven with respect to an operational semantics based on Markov decision processes. Our calculus preserves O'Hearn's frame rule, which enables local reasoning. We demonstrate that our calculus enables reasoning about quantities such as the probability of terminating with an empty heap, the probability of reaching a certain array permutation, or the expected length of a list.

==> case-study-putter-getter.tex <==
% !TEX root = ./main.tex


\subsection{Probabilistic Producer/Consumer} 

\begin{align*}
          \csPutGet\colon\quad
        & \WHILE{x \neq 0} \left\{ \qquad \left\{~
            \begin{aligned}
                    & \texttt{// $\csGet$} \\
                    & \ASSIGNH{y}{x}\SEMI \\
                    & \FREE{x}\SEMI \\
                    & \ASSIGN{x}{y}
            \end{aligned}
            ~\right\}\,\left[\sfrac{1}{2}\right]\,\left\{~
            \begin{aligned}
                    & \texttt{// $\csPut$} \\
                    & \ALLOC{x}{x}\SEMI \\
                    & \ALLOC{x}{x}\SEMI \\
                    & \ALLOC{x}{x} \\
                    %& \ProcCall{getLast}{x}{y}\SEMI \\
                    %& \ProcCall{produce}{3}{z}\SEMI \\
                    %& \ALLOC{z}{0}\SEMI\ALLOC{z}{z}\SEMI\ALLOC{z}{z} \\
                    %& \HASSIGN{y}{z}
            \end{aligned}
            ~\right\} \qquad \right\}
\end{align*}
%
Let us first note that program $\csPutGet$ is indeed memory safe if the input is a null-terminated list with head $x$, i.e.
%
\begin{align*}
  \wlp{\csPutGet}{\emp} \ssucceq \Ls{x}{0}.
\end{align*}
%
Now, how large is the probability that this system eventually runs out of produced goods?
\begin{align*}
        \wp{\csPutGet}{\emp} \eeq \frac{\sqrt{5}-1}{2} \cdot ???
\end{align*}
%

%\begin{align*}
%        & \ProcDecl{getLast}{x}{y} \\
%        & \qquad \ASSIGNH{z}{x}\SEMI\ASSIGN{y}{x} \\
%        & \qquad \WHILE{z \neq 0} \\
%        & \qquad \qquad \ASSIGN{y}{z}\SEMI \\
%        & \qquad \qquad \ASSIGNH{z}{x} \\
%        & \qquad \} \\
%        & \}
%\end{align*}

%\begin{align*}
%        & \ProcDecl{produce}{n}{z} \\
%        & \qquad \IF{n > 0} \\
%        & \qquad \qquad \ALLOC{z}{0}\SEMI \\
%        & \qquad \qquad \ASSIGN{n}{n-1}\SEMI;
%        & \qquad \qquad \WHILEDO{n > 0}{\ALLOC{z}{z}}
%        & \qquad \} \\
%        & \}
%\end{align*}




==> case-study-unsafe-list-traversal.tex <==
\subsection{Unsafe List Traversal}\label{sec:case-studies:unsafe-list-traversal}

\begin{align*}
          \csListTraverse\colon \quad
        & \WHILE{x \neq 0} \\
        & \qquad \ASSIGNH{y}{x}\SEMI \\
        & \qquad \PCHOICE{\ASSIGNH{y}{y}}{p}{\SKIP}\SEMI \\
        & \qquad \ASSIGN{x}{y} ~\}
\end{align*}

\begin{align*}
    \wp{\csListTraverse}{1} \eeq ?
\end{align*}


==> fig-landscape.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,node distance=2.5cm,semithick,minimum size=1cm]
\tikzstyle{every state}=[draw=none]
  %\draw[white, use as bounding box] (-1.1,-1.8) rectangle (6.4,1.5);
   \node [state, initial,outer sep=-1mm,initial text=] (init) {$\langle \cc,\, \sk,\, \hh \rangle$};


   \node (left) [left=1.2cm of init] {};
   \node [cloud, draw=black,cloud puffs=15, cloud puff arc= 135, outer sep=1mm, minimum width=1.5cm, minimum height=0.9cm, cloud ignores aspect] (fault) [above=0.0cm of left,outer sep=-1mm] {$\texttt{fault}$};
   \node [cloud, draw=black,cloud puffs=15, cloud puff arc= 135, outer sep=1mm, minimum width=1.5cm, minimum height=0.9cm, cloud ignores aspect] (diverge) [below=0.0cm of left,outer sep=-1mm] {diverge};

   \node (right) [right=1.2cm of init] {};
   \node [cloud, draw=black,cloud puffs=15, cloud puff arc= 135, outer sep=1mm, minimum width=1.5cm, minimum height=0.9cm, cloud ignores aspect] (f) [above=0.0cm of right, outer sep=-1mm] {$\ff$};
   \node [cloud, draw=black,cloud puffs=15, cloud puff arc= 135, outer sep=1mm, minimum width=1.5cm, minimum height=0.9cm, cloud ignores aspect] (nf) [below=0.0cm of right,outer sep=-1mm] {$1-\ff$};
   %\node [state] (sink) [right of=f,outer sep=-1mm] {$sink$};
   %\node [cloud, draw=black,cloud puffs=15, cloud puff arc= 150,
   %     minimum width=1.5cm, minimum height=.75cm, outer sep=1mm, aspect=1] (diverge) [below=0.5 cm of exit] {$\phantom{foo}$};

   % \node [] (divergetext) [below=-1 cm of diverge] {\small$diverge$};
  \path []
      (init) edge [decorate,decoration={snake, post length=5mm},shorten >=6pt] (f)
      (init) edge [decorate,decoration={snake, post length=5mm},shorten >=6pt] (fault)
      (init) edge [decorate,decoration={snake, post length=5mm},shorten >=6pt] (nf)
      (init) edge [decorate,decoration={snake, post length=5mm},shorten >=6pt] (diverge)
      %(f) edge [] (sink)
      %(fault.east) edge [shorten <=5pt] (sink)
      %(nf.east) edge [shorten <=5pt] (sink)
      %(sink) edge [loop right,looseness=6] (sink)
      (diverge) edge [loop left,decorate,looseness=8,decoration={snake, post length=4mm, pre length=4mm},shorten <=9pt,shorten >=8pt] (diverge);
\end{tikzpicture}
\caption{Schematic of possible executions of a probabilistic program (without nondeterminism).}
\label{fig:schematics}
\end{figure}




==> fig-lossy-reversal-invariant.tex <==
\begin{figure}[t]
\begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.0cm, decoration={brace,mirror,amplitude=7}]
                %thick,main node/.style={circle,,draw}
  %font=\sffamily\Large\bfseries,minimum size=1mm}]

  \begin{scope}
          \node (h1) [draw, circle] {};
          \node (h2) [draw, circle, right of=h1] {};
          \node (h3) [right of=h2] {$\ldots$};
          \node (h4) [draw, circle, right of=h3] {};
          
          \node (r1) [draw, circle, left of = h1] {};
          \node (r2) [draw, circle, left of=r1] {};
          \node (r3) [left of=r2] {$\ldots$};
          \node (r4) [draw, circle, left of=r3] {};

          \node (head) [above of = h1, node distance=0.6cm] {$\lsHead$};
          \node (rev) [above of = r1, node distance=0.6cm] {$\lsRev$};

  \path[->]
    (h1) edge (h2)
    (h2) edge (h3)
    (h3) edge (h4)
    (r1) edge (r2)
    (r2) edge (r3)
    (r3) edge (r4)
    ;
  
  \path
    (head) edge (h1)
    (rev) edge (r1)
  ;

  \draw [decorate] ([yshift=-5mm]h1.west) --node[below=3mm]{$\Len{\lsHead}{0}$} ([yshift=-5mm]h4.east);
  \draw [decorate] ([yshift=-5mm]r4.west) --node[below=3mm]{$\Len{\lsRev}{0}$} ([yshift=-5mm]r1.east);

  \end{scope}
\end{tikzpicture}
\caption{Illustration of the heap described by invariant $\inv$}
\label{fig:lossy-reversal-invariant}
\end{figure}

